MeetupNet Dublin: Discovering Communities in Dublin's Meetup Network

Meetup.com is a global online platform which facilitates the organisation of meetups in different parts of the world. A meetup group typically focuses on one specific topic of interest, such as sports, music, language, or technology. However, many users of this platform attend multiple meetups. On this basis, we can construct a co-membership network for a given location. This network encodes how pairs of meetups are connected to one another via common members. In this work we demonstrate that, by applying techniques from social network analysis to this type of representation, we can reveal the underlying meetup community structure, which is not immediately apparent from the platform's website. Specifically, we map the landscape of Dublin's meetup communities, to explore the interests and activities of meetup.com users in the city.

==> aics2018/table-centrality.tex <==
\begin{table}[!b]
\centering
\begin{subfigure}[t]{\textwidth}
\centering
\scriptsize{
\begin{tabular}{|r|p{6.5cm}|r|}
\hline
\textbf{Rank} & \textbf{Meetup Name}                                 & \textbf{Score} \\\hline
1             & Dublin Artificial Intelligence \& Deep Learning & 0.0659         \\
2             & Big Data Developers in Dublin                   & 0.0658         \\
3             & Data Scientists Ireland                         & 0.0654         \\
4             & Zalando Tech Events Dublin                      & 0.0651         \\
5             & Machine Learning Dublin                         & 0.0640         \\
6             & Data Science and Engineering Club               & 0.0639         \\
7             & Hackers and Founders Dublin                     & 0.0638         \\
8             & GDG Dublin                                      & 0.0635         \\
9             & Dublin Startup Founder 101                      & 0.0632         \\
10            & Dublin - Coder Forge                            & 0.0630    \\\hline    
\end{tabular}
}
\caption{Weighted eigenvector centrality}\label{tab:centrality_wec}
\end{subfigure}
%\vskip 2em
\begin{subfigure}[t]{\textwidth}
\centering
\scriptsize{
\begin{tabular}{|r|p{6.5cm}|r|}
\hline
\textbf{Rank} & \textbf{Meetup Name}                                    & \textbf{Score} \\\hline
1             & Speak English Dublin                               & 0.1053         \\
2             & AWS User Group Dublin                              & 0.0467         \\
3             & New and Not So New In Dublin                       & 0.0428         \\
4             & English Language Conversation with English Teacher & 0.0349         \\
5             & Events, Drinks and Dancing in Dublin               & 0.0327         \\
6             & Python Ireland                                     & 0.0323         \\
7             & Dublin UX                                          & 0.0289         \\
8             & Dublin Indoor Football at The Soccer Dome          & 0.0260         \\
9             & Dublin LGBT Social Meetup                          & 0.0229         \\
10            & Socializing Dublin                              & 0.0218 \\\hline       
\end{tabular}
}
\caption{Weighted betweenness centrality}\label{tab:centrality_wbc}
\end{subfigure}
\vskip 0.5em
\caption{Top 10 most central meetups in the Dublin meetup network, as ranked by (a) weighted eigenvector centrality and (b) weighted betweenness centrality.}
\label{tab:centrality}
\end{table}


% \begin{table}[]
% \begin{tabular}{lll}
% \textbf{Rank} & \textbf{Meetup}                                       & \textbf{Score} \\
% 1             & Zalando Tech Events Dublin                            & 16.70          \\
% 2             & The Dublin Mastermind Group for Growth \& Empowerment & 16.27          \\
% 3             & Dublin Artificial Intelligence \& Deep Learning       & 16.20          \\
% 4             & Tog Hackerspace                                       & 15.92          \\
% 5             & Dublin - Coder Forge                                  & 15.87          \\
% 6             & Dublin TED Talks Discussions                          & 15.78          \\
% 7             & Dublin Startup Founder 101                            & 15.77          \\
% 8             & CHAI Dublin (Chatbot \& AI) Meetup                    & 15.71          \\
% 9             & TechMeetup.space                                      & 15.65          \\
% 10            & Conscious Friendships                                 & 15.58         
% \end{tabular}
% \caption{Weighted degree}
% \label{my-label}
% \end{table}


==> aics2018/table-communities.tex <==
%!TEX root = main.tex
\begin{table}[!tb]
\centering
\scriptsize{
\begin{tabular}{|r|r|p{4.9cm}|p{4.9cm}|}
\hline\textbf{Id} & \textbf{Size} & \textbf{Name Label}                                                                                   & \textbf{Description Label}                                                                             \\\hline
5  & 216  & hiking, international, wicklow, friends, yoga, book, culture, adventure, language, travel             & fun, members, friends, time, hikes, free, social, friendly, looking, food                              \\
4  & 148  & meditation, yoga, healing, spiritual, heart, sound, empowerment, soul, life, positive                 & healing, life, meditation, experience, self, energy, practice, spiritual, mind, mindfulness            \\
7  & 137  & data, user, science, tech, engineering, big, cloud, users, things, learning                           & data, programming, developers, community, code, science, software, technology, technologies, learn     \\
17 & 118  & user, tech, security, cloud, sharepoint, technology, game, software, data, crypto                     & data, learn, share, learning, developers, cloud, community, security, technology, software             \\
14 & 84   & business, digital, marketing, startup, entrepreneurs, network, job, professionals, innovation, market & business, marketing, digital, entrepreneurs, startup, market, network, owners, sales, job              \\
22 & 80   & yoga, meditation, workshop, stress, dun, laoghaire, camino, running, dance, therapy                   & yoga, life, body, meditation, class, health, classes, practice, energy, mind                           \\
3  & 78   & startup, entrepreneurs, digital, lean, business, marketing, agile, growth, product, innovation        & business, entrepreneurs, marketing, startup, networking, digital, lean, product, community, innovation \\
25 & 77   & yoga, health, happiness, meditation, vegan, prayer, empowerment, circle, centre, self                 & yoga, life, meditation, help, support, healing, learn, world, health, work                             \\
10 & 71   & user, mysql, traders, developers, tech, js, product, data, sprint, net                                & learn, product, developers, mysql, share, community, meetups, professionals, technologies, engineers   \\
18 & 63   & music, singles, rock, social, travel, south, international, fans, electronic, 30s                     & music, night, friends, fun, singles, rock, singing, love, members, sing                                \\
8  & 61   & yoga, meditation, health, healing, classes, relaxation, self, body, light, sound                      & yoga, meditation, body, classes, life, mind, healing, health, practice, nature                         \\
21 & 54   & empowerment, self, book, support, health, workshop, eating, therapy, life, development                & life, world, diet, work, feel, learn, share, spiritual, ideas, find                                    \\
15 & 53   & circle, things, drinks, city, fun, hike, ladies, social, friends, book                                & drinks, friends, women, fun, book, food, wants, single, cinema, dinner                                 \\
16 & 53   & dance, dancing, yoga, classes, movement, salsa, fitness, class, set, handstand                        & dance, classes, dancing, fun, fitness, workout, 8pm, levels, class, movement                           \\
26 & 52   & soul, prayer, network, life, healing, workshop, empowerment, biodanza, centre, body                   & life, god, healing, faith, spiritual, love, evening, work, reiki, chat\\\hline                                
\end{tabular}
}
\vskip 0.5em
\caption{Summary of the 15 largest communities identified in the Dublin meetup network. Community labels are generated based on the top 10 terms appearing in the meetup name and description fields.}
\label{tab:comm}
\end{table}

==> aics2018/table-nodes.tex <==
%!TEX root = main.tex
\begin{table}[tb]
\centering
\scriptsize{
\begin{tabular}{|r|r|p{9.6cm}|}
\hline\textbf{Id} & \textbf{\% Over} & \textbf{Top 3 Meetups}\\\hline
5           & 16.7             & Kick Ass Adventures, Awesome Daytrips, Live Music  Artistic and Cultural Events \\
4           & 12.2             & Dublin Meditation Meetup, Dublin Self-Empowerment Coaching Meetup, Holistic Events Dublin \\
7           & 6.6              & Data Science and Engineering Club, Dublin Node.js Meetup, Dublin Artificial Intelligence \& Deep Learning \\
17          & 24.6             & Social Software Development Meetup in Dublin, Amazic Ireland: Enterprise Docker and DevOps, Fairy Tale Artificial General Intelligence Solutions \\
14          & 32.1             & Idea 2 Scale Dublin, SEO Strategy, Business Improvement \& Innovation Network \\
22          & 35.0               & Ki Yoga Massage, Dublin Wellness Meetup, Practical Ayurveda \\
3           & 34.6             & Startup Grind Dublin, Dublin Startup Founder 101, Start-Ed Dublin: Free legal forum for Startups \\
25          & 35.1             & Radical Forgiveness, Ki Yoga Massage, Dublin Grief Support Group \\
10          & 5.6              & WebRTC Meetup Ireland, Serverless-Dublin, NetDevOps Dublin \\
18          & 23.8             & Dublin Singles Party Meetup, Single Professionals Dublin, Dublin Nightlife \\
8           & 23.0               & Holistic Health and Wellness, Gentle Yoga, Beginner's Meditation Course \\
21          & 42.6             & Radical Forgiveness, Radical Human Expression, Dublin YouSA Meetup \\
15          & 5.7              & Finding things to do in Dublin, 40 (or almost) and fabulous, Random things to do in Dublin \\
16          & 26.4             & Stefano Argentine Tango, Samba Gafiera/Brazilian Zouk Dance Meetup, Dublin Dancing Meetup \\
26          & 25.0               & Healingoptions4u, Radical Forgiveness, Pilgrims' Prayer\\\hline               
\end{tabular}
}
\vskip 0.7em
\caption{The top 3 most central meetups in each of the 15 largest communities found. \emph{\% Over} shows the percentage of overlapping nodes in each community.}
\label{tab:nodes}
\end{table}
